Unleashing the Potential of Acquisition Functions in High-Dimensional Bayesian Optimization

Bayesian optimization (BO) is widely used to optimize expensive-to-evaluate black-box functions.BO first builds a surrogate model to represent the objective function and assesses its uncertainty. It then decides where to sample by maximizing an acquisition function (AF) based on the surrogate model. However, when dealing with high-dimensional problems, finding the global maximum of the AF becomes increasingly challenging. In such cases, the initialization of the AF maximizer plays a pivotal role, as an inadequate setup can severely hinder the effectiveness of the AF. This paper investigates a largely understudied problem concerning the impact of AF maximizer initialization on exploiting AFs' capability. Our large-scale empirical study shows that the widely used random initialization strategy often fails to harness the potential of an AF. In light of this, we propose a better initialization approach by employing multiple heuristic optimizers to leverage the historical data of black-box optimization to generate initial points for the AF maximize. We evaluate our approach with a range of heavily studied synthetic functions and real-world applications. Experimental results show that our techniques, while simple, can significantly enhance the standard BO and outperform state-of-the-art methods by a large margin in most test cases.

==> sections/3.1-background.tex <==

\subsection{Background}

BO is a class of machine-learning-based optimization methods to solve a black-box function optimization problem, $x^*=\argmin_x f(x)$, by attempting to find $x^*$ with the fewest samples. BO has two main components: a Bayesian
statistical surrogate model for modelling the objective function and an acquisition function (AF) for deciding where to
sample next. The surrogate model is typically implemented as a Gaussian process. It provides a Bayesian posterior
probability distribution that describes potential values for $f(x)$ at a candidate point $x$. The posterior distribution is updated each time we observe $f$ at a new sample point. For trading off exploitation and exploration,
the output of the surrogate model should contain both model prediction and uncertainty, constituting an AF. One prevalent AF\footnote{Other acquisition functions include the probability of improvement (PI) and expected improvement (EI).} is the
Upper Confidence Bound (UCB) function \cite{gpucb}, denoted as:
\begin{equation}
\alpha(x)=-\mu(x) + \sqrt{\beta_t}\cdot\sigma(x)
\end{equation}
where $\mu(x)$ and $\sigma(x)$ are the posterior mean (prediction) and posterior standard deviation (uncertainty) at point
$x$ predicted by the surrogate model, and $\beta_t$ is a hyperparameter that trades off between exploration and
exploitation. 

BO highly relies on fully maximizing the AF to uncover a global optimum, which is non-trivial for high-dimensional problems.  
However, very little work has investigated the quality of candidate samples generated during the AF maximization process and whether AF performs well in these candidates. 
In the following subsection, we present an example demonstrating that the commonly used random initialized AF maximization process restricts the potential of AF.







==> sections/3.2-motivation.tex <==
\subsection{Motivation}\label{3.2-motivation}

\begin{figure}[t]
    \centering  %图片全局居中
    \captionsetup[subfigure]{justification=centering}
    \begin{subfigure}{0.99\textwidth}
    \includegraphics[width=\textwidth]{figures//motivation-legend.pdf}
    \end{subfigure}
    
    % \begin{subfigure}{0.32\textwidth}
    % \centering    \includegraphics[width=\textwidth]{figures//motivation1-Ackley100.pdf}
    % \caption{}
    % \end{subfigure}
    % \hfill
    \begin{subfigure}{0.42\textwidth}
    \centering
    \includegraphics[width=\textwidth]{figures//motivation10-Ackley100.pdf}
    \caption{10 AF maximizer restarts}
    \end{subfigure}
    \hfill
    \begin{subfigure}{0.42\textwidth}
    \centering    \includegraphics[width=\textwidth]{figures//motivation1000-Ackley100.pdf}
    \caption{1000 AF maximizer restarts}
    \end{subfigure}
    
    
    
    % \vspace{0.2cm}

    \caption{Evaluating the sample chosen by AF-based selection against random and optimal selection among all intermediate candidate points generated during the AF maximization process when applying BO-grad to 100D Ackley functions. We use two random initialization settings for AF maximization: \textbf{(a)} 10 restarts and \textbf{(b)} 1000 restarts. In both settings, the performance of the native BO-grad (AF-based selection) is close to optimal selection and better than random selection, suggesting that the AF is effective at selecting a good sample from all candidates but is restricted by the pool of available candidates. Increasing the number of restarts from 10 to 1000 does not enhance the quality of intermediate candidates, indicating that a more effective initialization scheme, as opposed to random initialization, is necessary.}    \label{fig:motivation}
    
\end{figure}



As a motivation example, consider applying BO to optimize a 100-dimensional black-box Ackley function that is extensively used for testing optimization
algorithms. 
The goal is to find a set of input variables ($x$) to minimize the output, $f(x_1, \ldots, x_{100})$. 
The search domain is $-5 \leq x_i \leq 10, i= 1, 2, \ldots, 100$, with a global minimum of 0. For this example, we use a standard BO implementation with UCB ($\beta_t=1.96$) as the AF. Here, we use random search to create the initial starting points for a \emph{multi-start gradient-based} AF maximizer to iteratively generate multiple candidates, from which the AF chooses a sample for evaluation. In each BO iteration, we first evaluate the AF on  100000 random points and then select the top $n$ points as the initial points for the further gradient-based AF maximizer. We denote this implementation as \texttt{BO-grad}. In this example, we use two settings $n=10$ and $n=1000$.

As shown in Fig.~\ref {fig:motivation}(a), the function output given by BO-grad with 10 AF maximizer restarts is far from the global minimum of 0. We hypothesize that while the AF is effective, the low quality of candidate samples generated in AF maximization limits the power of the AF. To verify our hypothesis, we further consider two strategies: (1) either randomly select the next query point from all the candidate points generated during AF maximization or (2) exhaustively evaluate them at each BO iteration. The former and latter strategies correspond to ``\textbf{random selection}'' and ``\textbf{optimal selection}'' schemes, respectively. Despite the ideal but costly ``optimal selection'' search scenario, BO does not converge well, indicating intrinsic deficiencies in the AF maximization process. Meanwhile, the AF itself can choose a good candidate sample point to evaluate, as the performance of the native AF-based BO-grad is close to
that of ``optimal selection" and better than that of ``random selection". This observation suggests that the AF is effective at selecting a good sample in this case but its power is severely limited by the candidate samples generated during the AF maximization
process. We also observe similar results manifest when using other representative maximizers like random sampling and evolutionary algorithms. 

We then test what happens when we increase the number of AF maximization restarts of BO-grad to generate more candidates for AF to select at each iteration. However, in Fig.~\ref{fig:motivation}(b), it is evident that even with an increase in random restarts to 1000, the quality of intermediate candidate points generated during the AF maximization process remains similar to that with 10 restarts. Furthermore, in the case of 1,000 restarts, the performance of BO-grad is still close to that of ``optimal selection", reinforcing our observation that the pool of candidates restricts AF's power. This observation suggests that we need a better initialization scheme rather than simply increasing the number of restarts of random initialization.

This example motivates us to explore the possibility of improving the BO performance by providing the AF with better candidate samples through enhanced AF maximizer initialization. Our intuition is that the potential of AF is often not fully explored in HDBO. 
Moreover, the commonly used random initialization of the AF maximization process is often responsible for inferior candidates. We aim to improve the quality of the suggested samples through an enhanced mechanism for AF
maximizer initialization. As we will show in Section \ref {sec:results}, our strategy significantly improves BO on the 100D Ackley function, finding an output minimum of less than 0.5, compared to 6 given by BO-grad after evaluating 5,000 samples.
